Shape: A 3D Modeling Tool for Astrophysics

We present a flexible interactive 3D morpho-kinematical modeling application for astrophysics. Compared to other systems, our application reduces the restrictions on the physical assumptions, data type and amount that is required for a reconstruction of an object's morphology. It is one of the first publicly available tools to apply interactive graphics to astrophysical modeling. The tool allows astrophysicists to provide a-priori knowledge about the object by interactively defining 3D structural elements. By direct comparison of model prediction with observational data, model parameters can then be automatically optimized to fit the observation. The tool has already been successfully used in a number of astrophysical research projects.

==> Makefile <==
FILENAME = shape
LATEX = pdflatex #--interaction batchmode

# in order to create a .pdf from an .eps file, run epstopdf $EPSFILE -o=${EPSFILE%.eps}.pdf

PDFVIEWER = $(shell if [ `uname` = 'Linux' ]; then\
			echo 'acroread'; \
			else \
			echo 'open'; \
			fi \
			)

run: $(FILENAME)-small.pdf
	$(PDFVIEWER) $(FILENAME)-small.pdf &

quick:
	$(LATEX) $(FILENAME).tex
	$(PDFVIEWER) $(FILENAME).pdf &

$(FILENAME)-small.pdf: $(FILENAME).pdf
	gs -sDEVICE=pdfwrite -dNOPAUSE -dBATCH -dPDFSETTINGS=/ebook -sOutputFile=$@ $<

$(FILENAME).pdf: $(FILENAME).tex $(FILENAME).bbl
	$(LATEX) $(FILENAME).tex && $(LATEX) $(FILENAME).tex

$(FILENAME).bbl: $(FILENAME).aux shape.bib
	$(LATEX) $(FILENAME).tex && bibtex $(FILENAME).aux

$(FILENAME).aux: $(FILENAME).tex shape.bib
	$(LATEX) $(FILENAME).tex

.PHONY:
clean:
	@rm -f *.ps *.dvi *.log *.blg *.aux *.toc *.bbl *.out chapters/*.aux chapters/*.log *~ chapters/*~ *.backup chapters/*.backup

.PHONY:
purge:
	@rm -f *.ps *.dvi *.log *.blg *.aux *.toc *.bbl *.out chapters/*.aux chapters/*.log *~ chapters/*~ *.backup chapters/*.backup $(FILENAME).pdf $(FILENAME)-small.pdf


